Semi-Generative Modelling: Covariate-Shift Adaptation with Cause and Effect Features

Current methods for covariate-shift adaptation use unlabelled data to compute importance weights or domain-invariant features, while the final model is trained on labelled data only. Here, we consider a particular case of covariate shift which allows us also to learn from unlabelled data, that is, combining adaptation with semi-supervised learning. Using ideas from causality, we argue that this requires learning with both causes, $X_C$, and effects, $X_E$, of a target variable, $Y$, and show how this setting leads to what we call a semi-generative model, $P(Y,X_E|X_C,\theta)$. Our approach is robust to domain shifts in the distribution of causal features and leverages unlabelled data by learning a direct map from causes to effects. Experiments on synthetic data demonstrate significant improvements in classification over purely-supervised and importance-weighting baselines.

==> conclusion.tex <==
We have developed a novel framework for semi-supervised learning under changes in the distribution of input (or causal) features resulting from domain shift. 
This approach is suitable for domain adaptation problems for which the causal structure is known and for which the amount of labelled data is the main limitation, so that benefits from improving the supervised model outweigh the adaptation task.
 Our semi-generative model $P(Y, X_E\,|\,X_C)$ for learning with cause and effect features is inspired by recent work on independent mechanisms, and does not require self-training or expectation maximisation.
Rather it directly imposes constraints on the supervised model by learning a map from causes to effects from unlabelled data. 
Our analysis and empirical results suggest that this unsupervised model needs to be sufficiently constrained in order to improve estimates of the mechanisms $P(Y\,|\,X_C)$ and $P(X_E\,|\,Y)$ without supervision. 
For too flexible models, on the other hand, overfitting of unlabelled data can result in deteriorated performance. 
Our approach thus works best for classification where we have demonstrated significant improvements over the supervised baseline, importance-reweighting, and feature-transformation methods on synthetic data sets when only very few labelled training examples are available.
Moreover, on a domain-adaptation regression problem for protein signalling networks we have shown that our method can be beneficial also on real-world data, even when the underlying causal assumptions are no longer strictly satisfied. Especially in this context, it is useful that background and expert knowledge can easily be integrated in our modelling framework---something which is not straight-forward when using a feature tranformations approach to domain adaptation.
